Evaluating Communicative Success in Machine-Translated Conversation

Interpreter agents built on machine translation (MT) increasingly mediate live conversation, yet existing MT metrics cannot measure whether the translated message is understood and enables communication. We introduce a reusable, context-grounded checklist framework that evaluates interpreter-mediated text conversation across semantic, pragmatic, and cultural-social layers, capturing aspects missed by conventional MT metrics to serve as a closer proxy to evaluate communicative success. The framework supports both single-turn evaluation and interactive multi-turn simulations, scoring individual turns alongside overall conversational outcomes. We validate our approach via human validation, controlled perturbations, and cross-judge comparisons. Using this framework, we benchmark 10 interpreter setups across Arabic, Bengali, Indonesian, and Korean, covering 6,000 OpenSubtitles scenarios in 12 single-turn directions and multi-turn dialogues across all 6 language pairs. Under the main judge and two independent checklist generators, pragmatic and cultural-social criteria are harder than semantic, while conventional metrics overlook critical failures among stronger interpreters. Finally, prompt ablations show that scenario context and cultural adaptation drive LLM advantages over dedicated MT models. Together, our framework and benchmark offer a more faithful, communication-grounded proxy for evaluating conversational interpreter agents.

==> sections/07_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{The interpreter setup is the unit of evaluation.}
Context access, translation brief, and decoding interface together shape what an interpreter
achieves. Changing only the brief moves the pooled pass rate of the same seven setups by 14.9
points (Table~\ref{tab:prompt-ablation}), and without context and brief the LLMs score at the level
of Google Translate and NLLB-200. Benchmarks of interpreter agents should report the complete setup
together with the model name.

\paragraph{Relative and absolute pass rates.}
Our validation supports comparing setups under the same judge. Absolute pass rates need more
care: cascading human--judge agreement to the full dataset shows that the judge under-scores by up
to 18.8 points in three of four languages (Appendix~\ref{sec:appendix-cascade}), so absolute rates
require human calibration before serving as deployment thresholds.


==> tables/mt_metric_blindspots.tex <==
\begin{table}[!ht]
  \centering
  \caption{Disagreement on 5,624 Gemini 3.1 Pro outputs. The middle column is the percentage of
  each metric's top quartile with communicative pass rate at most 0.6. The final column is the
  percentage of its bottom quartile with communicative pass rate at least 0.9.}
  \label{tab:mt-metric-blindspots}
  \small
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{Metric} & \textbf{Top-rated outputs that fail}
      & \textbf{Bottom-rated outputs that pass} \\
    \midrule
    CometKiwi (QE) & 10.7\% & 62.0\% \\
    GEMBA-MQM      & 11.7\% & 67.5\% \\
    MQM-APE        & 12.2\% & 69.6\% \\
    RATE           & 10.3\% & 62.2\% \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/multiturn_consistency_gap.tex <==
\begin{table}[htbp]
  \centering
  \caption{Conversation-level minus mean turn-level success, setups with a significant gap
  (Holm-uncorrected paired bootstrap, full table in \texttt{data/q3\_consistency\_gap.csv}).
  Indonesian--Korean is the one pair where conversation-level scoring is consistently
  \emph{higher}, and every other pair with a significant gap shows the opposite sign, except
  $^\dagger$Tiny Aya on Arabic--Bengali, which alone reverses ar-bn's otherwise-negative pattern. No
  setup on any pair shows a declining turn-success trend across turn index 0--5
  (Figure~\ref{fig:multiturn-turn-index}).}
  \label{tab:multiturn-consistency-gap}
  \small
  \begin{tabular}{@{}lrl@{}}
    \toprule
    \textbf{Pair} & \textbf{Sig.\ setups} & \textbf{Conv.\ $-$ turn range} \\
    \midrule
    Indonesian--Korean & 6/9 & $+0.7$ to $+6.3$ pts \\
    Arabic--Bengali    & 5/5 & $-6.2$ to $+10.5$ pts$^\dagger$ \\
    Arabic--Korean     & 8/9 & $-14.6$ to $-2.3$ pts \\
    Bengali--Indonesian & 4/5 & $-15.1$ to $-2.2$ pts \\
    Bengali--Korean    & 1/5 & $-15.7$ pts (Tiny Aya only) \\
    Arabic--Indonesian & 0/5 & none significant \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/multiturn_context.tex <==
\begin{table}[t]
  \centering
  \caption{Effect of translated history on real scripted dialogue: Flash Lite with minus without history (points), 100 conversations per pair. Every pair is significant ($p<0.001$).}
  \label{tab:multiturn-context}
  \small
  \setlength{\tabcolsep}{2pt}
  \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccccc@{}}
    \toprule
    \textbf{Pair} & Bn--Ko & Id--Ko & Ar--Bn & Ar--Id & Ar--Ko & Bn--Id \\
    \midrule
    $\Delta$ turn level & $+5.3$ & $+4.5$ & $+4.2$ & $+4.0$ & $+3.9$ & $+3.5$ \\
    \bottomrule
  \end{tabular*}
\end{table}


==> tables/multiturn_guided_vs_free.tex <==
\begin{table}[htbp]
  \centering
  \caption{Holm-significant guided--free conversation-level differences (3/12
  setup$\times$pair comparisons), with $\Delta$ = guided $-$ free.}
  \label{tab:multiturn-guided-vs-free}
  \small
  \resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
  \begin{tabular}{@{}llrrrl@{}}
    \toprule
    \textbf{Pair} & \textbf{Setup} & \textbf{Guided} & \textbf{Free} & \textbf{$\Delta$} & \textbf{Sig.} \\
    \midrule
    Arabic--Bengali & Flash Lite & 0.875 & 0.963 & $-8.9$pts & yes \\
    Arabic--Korean  & Flash Lite & 0.871 & 0.964 & $-9.3$pts & yes \\
    Bengali--Indonesian & Flash Lite & 0.897 & 0.980 & $-8.3$pts & yes \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/multiturn_overview.tex <==
\begin{table}[t]
  \centering
  \caption{Multi-turn pass rates pooled over the 6 pairs: single-turn level in the same directions, turn level, and whole conversation. Per-pair results are in Appendix~\ref{sec:appendix-multiturn-pilot}.}
  \label{tab:multiturn-overview}
  \small
  \setlength{\tabcolsep}{3pt}
  \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lccc@{}}
    \toprule
    \textbf{Setup} & \textbf{Single} & \textbf{Turn} & \textbf{Conv.} \\
    \midrule
    \multicolumn{4}{@{}l}{\emph{Real scripted dialogue}} \\
    Flash Lite, history    & 74.0 & 77.7 & 81.5 \\
    Qwen3.5 Flash          & 74.0 & 75.8 & 77.1 \\
    Flash Lite, no history & 74.0 & 73.5 & 73.2 \\
    NLLB-200               & 53.0 & 60.9 & 58.7 \\
    Tiny Aya               & 49.5 & 57.8 & 53.2 \\
    \midrule
    \multicolumn{4}{@{}l}{\emph{Dynamic conversation}} \\
    Flash Lite             & -- & 84.6 & 89.0 \\
    Qwen3.5 Flash          & -- & 83.2 & 87.8 \\
    \bottomrule
  \end{tabular*}
\end{table}


==> tables/multiturn_scripted_ranking.tex <==
\begin{table}[htbp]
  \centering
  \caption{Scripted-mode mean turn-level success rate, canonical 5-setup roster, all 6 pairs (118--125
  six-turn conversations per setup per pair, 708--750 turns each). The two LLM interpreters cluster
  tightly (0.87--0.97), while the dedicated-MT floor (NLLB-200) and the tiny generalist (Tiny Aya) trail by
  30--50 points on every pair.}
  \label{tab:multiturn-scripted-ranking}
  \small
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    \textbf{Pair} & \textbf{Flash Lite+ctx} & \textbf{Flash Lite noctx} & \textbf{Qwen3.5 Flash} & \textbf{NLLB-200 (floor)} & \textbf{Tiny Aya (floor)} \\
    \midrule
    Arabic--Bengali    & 0.959 & 0.947 & 0.945 & 0.570 & 0.379 \\
    Arabic--Indonesian & 0.895 & 0.870 & 0.870 & 0.449 & 0.643 \\
    Arabic--Korean     & 0.957 & 0.946 & 0.940 & 0.411 & 0.523 \\
    Bengali--Indonesian & 0.924 & 0.909 & 0.901 & 0.494 & 0.400 \\
    Bengali--Korean    & 0.955 & 0.947 & 0.929 & 0.413 & 0.336 \\
    Indonesian--Korean & 0.966 & 0.965 & 0.951 & 0.365 & 0.547 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/multiturn_scripted_vs_dynamic.tex <==
\begin{table}[htbp]
  \centering
  \caption{Holm-significant scripted--dynamic turn-level differences (4/12
  setup$\times$pair comparisons), with $\Delta$ = scripted $-$ dynamic. The samples are unpaired
  because they use different conversations.}
  \label{tab:multiturn-scripted-vs-dynamic}
  \small
  \resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
  \begin{tabular}{@{}llrrrl@{}}
    \toprule
    \textbf{Pair} & \textbf{Setup} & \textbf{Scripted} & \textbf{Dynamic} & \textbf{$\Delta$} & \textbf{Sig.} \\
    \midrule
    Arabic--Indonesian & Flash Lite+ctx & 0.895 & 0.933 & $-3.8$pts & yes \\
    Arabic--Indonesian & Qwen3.5 Flash  & 0.870 & 0.927 & $-5.7$pts & yes \\
    Bengali--Indonesian & Qwen3.5 Flash & 0.901 & 0.932 & $-3.2$pts & yes \\
    Indonesian--Korean & Qwen3.5 Flash  & 0.951 & 0.969 & $-1.8$pts & yes \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/multiturn_vs_single.tex <==
\begin{table}[htbp]
  \centering
  \caption{Mean per-direction difference between multi-turn (no-context) and matching single-turn
  success, averaged over 12 directions. Figure~\ref{fig:multiturn-ranking-scatter} shows the
  per-direction values.}
  \label{tab:multiturn-vs-single}
  \small
  \resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
  \begin{tabular}{@{}lrr@{}}
    \toprule
    \textbf{Setup} & \textbf{Mean $\Delta$ (multi $-$ single)} & \textbf{$n$ directions} \\
    \midrule
    Flash Lite, no context & +16.1 pts & 12 \\
    Qwen3.5 Flash          & +15.6 pts & 12 \\
    Tiny Aya                    & +2.7 pts  & 12 \\
    NLLB-200 3.3B           & $-$4.5 pts & 12 \\
    \bottomrule
  \end{tabular}}
\end{table}

